Device-Agnostic Millimeter Wave Beam Selection using Machine Learning

Most research in the area of machine learning-based user beam selection considers a structure where the model proposes appropriate user beams. However, this design requires a specific model for each user-device beam codebook, where a model learned for a device with a particular codebook can not be reused for another device with a different codebook. Moreover, this design requires training and test samples for each antenna placement configuration/codebook. This paper proposes a device-agnostic beam selection framework that leverages context information to propose appropriate user beams using a generic model and a post processing unit. The generic neural network predicts the potential angles of arrival, and the post processing unit maps these directions to beams based on the specific device's codebook. The proposed beam selection framework works well for user devices with antenna configuration/codebook unseen in the training dataset. Also, the proposed generic network has the option to be trained with a dataset mixed of samples with different antenna configurations/codebooks, which significantly eases the burden of effective model training.

==> Rotation/Rotation_code.tex <==
\iffalse
    \begin{figure}[t]
\centering
\tdplotsetmaincoords{70}{130}
\begin{tikzpicture}[tdplot_main_coords, scale=1]

\draw[>=latex',  ->, line width  = 1pt] (0,0,0) -- ++ (2.9,0,0) node[left =-1pt]{$x$};  % X axis (AP)
\draw[>=latex',  ->, line width  = 1pt] (0,0,0) -- ++ (0,1.5,0) node[right=-1pt]{$y$};  % Y axis (AP)
\draw[>=latex',  ->, line width  = 1pt] (0,0,0) -- ++ (0,0,1.5) node[above=-1pt]{$z$};  % Z axis (AP)

\begin{scope}[rotate around z=15] % 15
    \begin{scope}[rotate around x=25] % 25
        \begin{scope}[shift={(1.236,0, 0.29)}]. % 7/6cos(10)+0.5sin(10), -7/6sin(10)+0.5cos(10)
            \draw[>=latex', dashed, line width  = 1pt] (0,0,0) -- ++ (0,0,1) node[above=-1pt]{};  % axis
            \draw[blue, dashed, opacity=0.8] (-7/6,0,-0.5) -- ++(7/3,0,0) -- ++(0,0,1) -- ++(-7/3,0,0) -- cycle;
            \begin{scope}[rotate around y=10] % 10
                \draw[blue, fill=blue, opacity=0.2] (-7/6,0,-0.5) -- ++(7/3,0,0) -- ++(0,0,1) -- ++(-7/3,0,0) -- cycle;
                %\draw[blue, fill=blue, opacity=0.1] (-2,0,-1) -- ++(6,0,0) -- ++(0,0,2) -- ++(-6,0,0) -- cycle; % plane
                \draw[>=latex', line width  = 1pt] (0,0,0) -- ++ (0,0,0.96) node[above=-1pt]{};  % rotated axis
                
                \draw[blue, opacity=0.2] (1/3-7/6,0,-0.5) -- ++(0,0,1) -- ++(1/3,0,0) -- ++(0,0,-1) -- ++(1/3,0,0) -- ++(0,0,1) -- ++(1/3,0,0) -- ++(0,0,-1)
                -- ++(1/3,0,0) -- ++(0,0,1) -- ++(1/3,0,0) -- ++(0,0,-1)
                -- ++(1/3,0,0) -- ++(0,0,1) ;
                
                \draw[blue, opacity=0.2] (-7/6,0,1/3-0.5) -- ++(7/3,0,0) -- ++(0,0,1/3) -- ++(-7/3,0,0) -- ++(0,0,1/3) -- ++(7/3,0,0) ;
                
                \foreach \i in {0,...,7} {
                    \foreach \j in {0,...,3} {
                        % \filldraw[blue] (\i/3,0,\j/3) circle (1.5pt);
                        \draw[blue, >=triangle 45,  ->, line width  = .1pt] (\i/3-7/6,0,\j/3-0.5) -- (\i/3-7/6,0,\j/3-0.6);
                } 
                }
            \end{scope}
            \tdplotgetpolarcoords{1}{0}{1}
            \tdplotsetthetaplanecoords{\tdplotresphi}
            \tdplotdrawarc[>=latex', -, line width=0.5pt, tdplot_rotated_coords]{(0,0,0)}{1.25}{27}{32}{anchor=south, xshift=-0pt}{$\beta_{t}$}
        \end{scope}
    \end{scope}
\end{scope}

\tdplotdrawarc[>=latex', <->, line width=0.5pt] {(0, 0, 0)} {7/3}{0}{15}{anchor=north}{$\alpha_{t}$};
\tdplotgetpolarcoords{0.1}{-.5}{1}
\tdplotsetthetaplanecoords{\tdplotresphi}
\tdplotdrawarc[>=latex', <->, line width=0.5pt, tdplot_rotated_coords]{(0,0,0)}{0.9}{0}%
{35}{anchor=south, xshift=-0pt}{$\gamma_{t}$}


\begin{scope}[shift={(1,7,3)}]
    \draw[>=latex',  ->, line width  = 1pt] (0,0,0) -- ++ (2.9,0,0) node[left =-1pt]{$x$};  % X axis (AP)
    \draw[>=latex',  ->, line width  = 1pt] (0,0,0) -- ++ (0,1.5,0) node[right=-1pt]{$y$};  % Y axis (AP)
    \draw[>=latex',  ->, line width  = 1pt] (0,0,0) -- ++ (0,0,1.5) node[above=-1pt]{$z$};  % Z axis (AP)
    \begin{scope}[rotate around z=60]
        \begin{scope}[rotate around x=-40]
        \begin{scope}[shift={(1.256,0, 0.18)}]. % 7/6cos(10)+0.5sin(10), -7/6sin(10)+0.5cos(10)
            \draw[>=latex', dashed, line width  = 1pt] (0,0,0) -- ++ (0,0,1) node[above=-1pt]{};  % axis
            \draw[magenta, dashed, opacity=0.8] (-7/6,0,-0.5) -- ++(7/3,0,0) -- ++(0,0,1) -- ++(-7/3,0,0) -- cycle;
            \begin{scope}[rotate around y=15] % 10
                \draw[magenta, fill=magenta, opacity=0.2] (-7/6,0,-0.5) -- ++(7/3,0,0) -- ++(0,0,1) -- ++(-7/3,0,0) -- cycle;
                
                \draw[>=latex', line width  = 1pt] (0,0,0) -- ++ (0,0,0.95) node[above=-1pt]{};  % rotated axis
                
                \draw[magenta, opacity=0.2] (1/3-7/6,0,-0.5) -- ++(0,0,1) -- ++(1/3,0,0) -- ++(0,0,-1) -- ++(1/3,0,0) -- ++(0,0,1) -- ++(1/3,0,0) -- ++(0,0,-1)
                -- ++(1/3,0,0) -- ++(0,0,1) -- ++(1/3,0,0) -- ++(0,0,-1)
                -- ++(1/3,0,0) -- ++(0,0,1) ;
                
                \draw[magenta, opacity=0.2] (-7/6,0,1/3-0.5) -- ++(7/3,0,0) -- ++(0,0,1/3) -- ++(-7/3,0,0) -- ++(0,0,1/3) -- ++(7/3,0,0) ;
                \foreach \i in {0,...,7} {
                    \foreach \j in {0,...,3} {
                        %\filldraw[magenta] (\i/3,0,\j/3) circle (1.5pt);
                        \draw[magenta, >=triangle 45,  ->, line width  = .1pt] (\i/3-7/6,0,\j/3-0.5) -- (\i/3-7/6,0,\j/3-0.6);
                } 
                }
            \end{scope}
            \tdplotgetpolarcoords{1}{0}{1}
            \tdplotsetthetaplanecoords{\tdplotresphi}
            \tdplotdrawarc[>=latex', -, line width=0.5pt, tdplot_rotated_coords]{(0,0,0)}{1.05}{292}{300}{anchor=south, xshift=5pt}{$\beta_{r}$}
        \end{scope}
        \end{scope}
    \end{scope}
    \tdplotdrawarc[>=latex', <->, line width=0.5pt] {(0, 0, 0)} {7/3}{0}{60}{anchor=north}{$\alpha_{r}$};
    \tdplotgetpolarcoords{-0.6}{0.5}{1}
    \tdplotsetthetaplanecoords{\tdplotresphi}
    \tdplotdrawarc[>=latex', <->, line width=0.5pt, tdplot_rotated_coords]{(0,0,0)}{0.9}{0}%
    {45}{anchor=south, xshift=1pt}{$\gamma_{r}$}
\end{scope}

\end{tikzpicture}
\caption{The dashed rectangles show the arrays before rotating about the $y$-axis}
\label{SystemModel}
\end{figure}
\fi

\begin{figure}[t]
\centering
\tdplotsetmaincoords{70}{130}
\begin{tikzpicture}[tdplot_main_coords, scale=1]

\draw[>=latex',  ->, line width  = 1pt] (0,0,0) -- ++ (2.9,0,0) node[left =-1pt]{$x$};  % X axis (AP)
\draw[>=latex',  ->, line width  = 1pt] (0,0,0) -- ++ (0,1.5,0) node[right=-1pt]{$y$};  % Y axis (AP)
\draw[>=latex',  ->, line width  = 1pt] (0,0,0) -- ++ (0,0,1.5) node[above=-1pt]{$z$};  % Z axis (AP)

%\begin{scope}[rotate around z=20] % 15
%    \begin{scope}[rotate around x=25] % 25
%        \begin{scope}[shift={(1.26,0, -0.15)}]. % 7/6cos(30)+0.5sin(30), -7/6sin(30)+0.5cos(30)
%            \begin{scope}[rotate around y=30] % 10
\begin{scope}[shift={(1.55,0.5, -0.15)}]. % 7/6cos(30)+0.5sin(30), -7/6sin(30)+0.5cos(30)            
    \begin{scope}[rotate around z=20] % 15
        \begin{scope}[rotate around y=30] % 25
            \begin{scope}[rotate around x=25] % 10
                \draw[blue, fill=blue, opacity=0.2] (-7/6,0,-0.5) -- ++(7/3,0,0) -- ++(0,0,1) -- ++(-7/3,0,0) -- cycle;
                \draw[blue, opacity=0.2] (1/3-7/6,0,-0.5) -- ++(0,0,1) -- ++(1/3,0,0) -- ++(0,0,-1) -- ++(1/3,0,0) -- ++(0,0,1) -- ++(1/3,0,0) -- ++(0,0,-1)
                -- ++(1/3,0,0) -- ++(0,0,1) -- ++(1/3,0,0) -- ++(0,0,-1)
                -- ++(1/3,0,0) -- ++(0,0,1) ;
                
                \draw[blue, opacity=0.2] (-7/6,0,1/3-0.5) -- ++(7/3,0,0) -- ++(0,0,1/3) -- ++(-7/3,0,0) -- ++(0,0,1/3) -- ++(7/3,0,0) ;
                
                \foreach \i in {0,...,7} {
                    \foreach \j in {0,...,3} {
                        % \filldraw[blue] (\i/3,0,\j/3) circle (1.5pt);
                        \draw[blue, >=triangle 45,  ->, line width  = .1pt] (\i/3-7/6,0,\j/3-0.5) -- (\i/3-7/6,0,\j/3-0.6);
                } 
                }
                
                \draw[>=latex', dashed, ->, line width  = 1pt] (0,0,0) -- ++ (1.5,0,0) node[below left=-3pt and -7.5pt]{$\dddot{x}$};  % rotated axis x
                \draw[>=latex', dashed, ->, line width  = 1pt] (0,0,0) -- ++ (0,1.5,0) node[above right=-5pt and -5pt]{$\dddot{y}$};  % rotated axis y
                \draw[>=latex', dashed, ->, line width  = 1pt] (0,0,0) -- ++ (0,0,1.5) node[above left=-5pt and -5pt]{$\dddot{z}$};  % rotated axis z
            \end{scope}
        \end{scope}
    \end{scope}
\end{scope}
\end{tikzpicture}
%\caption{}
%\label{SystemModel}
%\end{figure}

%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%

%\begin{figure}[t]
\centering
\tdplotsetmaincoords{70}{130}
\begin{tikzpicture}[tdplot_main_coords, scale=1]
\fill[red!50,opacity=0.3] (0,-1.5,-1.5) -- (0,1.5,-1.5) -- (0,1.5,1.5) -- (0,-1.5,1.5) -- (0,-1.5,-1.5);
\draw[>=latex',  ->, line width  = 1pt] (0,0,0) -- ++ (2.5,0,0) node[above left = -12pt and -25pt]{$x, \dot{x}$ \hspace{5pt} \AxisRotator[x=0.2cm,y=0.3cm, rotate=0, violet]};  % X axis (AP)
\draw[>=latex',  ->, line width  = 1pt] (0,0,0) -- ++ (0,1.5,0) node[right=-1pt]{$y$};  % Y axis (AP)
\draw[>=latex',  ->, line width  = 1pt] (0,0,0) -- ++ (0,0,1.5) node[above=-1pt]{$z$};  % Z axis (AP)

\begin{scope}[rotate around x=25] % 25
    \draw[>=latex', loosely dotted, ->, line width  = 1pt] (0,0,0) -- ++ (0,1.5,0) node[right=-1pt]{$\dot{y}$};  % Y axis (AP)
    \draw[>=latex', loosely dotted, ->, line width  = 1pt] (0,0,0) -- ++ (0,0,1.5) node[above=-1pt]{$\dot{z}$};  % Z axis (AP)
\end{scope}


\tdplotgetpolarcoords{0.1}{-.5}{1}
\tdplotsetthetaplanecoords{\tdplotresphi}
\tdplotdrawarc[>=latex', <->, line width=0.5pt, tdplot_rotated_coords]{(0,0,0)}{0.9}{0}%
{25}{anchor=south, xshift=-0pt}{\footnotesize $\gamma_{r}$}


\begin{scope}[shift={(-4,4,0)}]
    \begin{scope}[rotate around x=25] % 25
        \fill[red!50,opacity=0.3] (-1.5,0,-1.5) -- (1.5,0,-1.5) -- (1.5,0,1.5) -- (-1.5,0,1.5) -- (-1.5,0,-1.5);
        \draw[>=latex', loosely dotted, ->, line width  = 1pt] (0,0,0) -- ++ (1.5,0,0) node[left =-1pt]{$\dot{x}$};  % X axis (AP)
        \draw[>=latex', loosely dotted, ->, line width  = 1pt] (0,0,0) -- ++ (0,2.5,0) node[above right=-5pt and -2pt]{$\dot{y}, \ddot{y}$};  % Y axis (AP)
        \draw[>=latex', loosely dotted, ->, line width  = 1pt] (0,0,0) -- ++ (0,2.5,0) node[above right=-20pt and -30pt]{\AxisRotator[x=0.2cm,y=0.3cm, rotate=10, solid, violet]}; 
        \draw[>=latex', loosely dotted, ->, line width  = 1pt] (0,0,0) -- ++ (0,0,1.5) node[above=-1pt]{$\dot{z}$};  % Z axis (AP)
        \draw[>=latex', densely dotted, ->, line width  = 1pt] (0,0,0) -- ++ (0,2.5,0) node[right=-1pt]{};  % Y axis (AP)
    \end{scope}
    \begin{scope}[rotate around y=30] % 10
        \begin{scope}[rotate around x=25] % 25
            \draw[>=latex', densely dotted, ->, line width  = 1pt] (0,0,0) -- ++ (1.3,0,0) node[below right = -2pt and -9pt]{$\ddot{x}$};  % X axis (AP)
            
            \draw[>=latex', densely dotted, ->, line width  = 1pt] (0,0,0) -- ++ (0,0,1.5) node[above=-1pt]{$\ddot{z}$};  % Z axis (AP)
        \end{scope}

    \end{scope}
    \tdplotgetpolarcoords{1}{0}{0}
    \tdplotsetthetaplanecoords{\tdplotresphi}
    \tdplotdrawarc[>=latex', <->, line width=0.5pt, tdplot_rotated_coords]{(0,0,0)}{0.9}{90}%
    {120}{xshift=-5pt, yshift=-4pt}{\footnotesize $\beta_{r}$}
\end{scope}


\begin{scope}[shift={(-8,8,0)}]
    \begin{scope}[rotate around y=30] % 25
        \begin{scope}[rotate around x=25] 
            \fill[red!50,opacity=0.3] (-1.5,-1.5,0) -- (1.5,-1.5,0) -- (1.5,1.5,0) -- (-1.5,1.5,0) -- (-1.5,-1.5,0);
            \draw[>=latex', densely dotted, ->, line width  = 1pt] (0,0,0) -- ++ (1.5,0,0) node[left =-1pt]{$\ddot{x}$};  % X axis (AP)
            \draw[>=latex', densely dotted, ->, line width  = 1pt] (0,0,0) -- ++ (0,1.5,0) node[right=-1pt]{$\ddot{y}$};  % Y axis (AP)
            \draw[>=latex', densely dotted, ->, line width  = 1pt] (0,0,0) -- ++ (0,0,1.5) node[above=-1pt]{$\ddot{z}, \dddot{z}$};  % Z axis (AP)
            \draw[>=latex', loosely dotted, ->, line width  = 1pt] (0,0,0) -- ++ (0,0,1.5) node[above right=-25pt and 0pt]{\AxisRotator[x=0.2cm,y=0.3cm, rotate=100, solid, violet]}; 
        \end{scope}
    \end{scope}
    
    \begin{scope}[rotate around z=20]
        \begin{scope}[rotate around y=30] % 25
            \begin{scope}[rotate around x=25] 
                \draw[>=latex', dashed, ->, line width  = 1pt] (0,0,0) -- ++ (1.3,0,0) node[below=0pt]{$\dddot{x}$};  % X axis (AP)
                \draw[>=latex', dashed, ->, line width  = 1pt] (0,0,0) -- ++ (0,0,1.5) node[above=-1pt]{};  % Z axis (AP)
                
                \tdplotdrawarc[>=latex', <->, line width=0.5pt] {(0, 0, 0)} {1.2}{0}{-20}{below right =-5pt and -5pt}{$\alpha_{r}$};
            \end{scope}
        \end{scope}
    \end{scope}
    
    \begin{scope}[rotate around z=70]
        \begin{scope}[rotate around y=30] % 25
            \begin{scope}[rotate around x=25] 
            
            \draw[>=latex', dashed, ->, line width  = 1pt] (0,0,0) -- ++ (0,1,0) node[above=2pt]{$\dddot{y}$};  % Y axis (AP)
            
            \end{scope}
        \end{scope}
    \end{scope}
    
\end{scope}


\end{tikzpicture}
\caption{By rotating around the $x$, $y$, and $z$ axes, a transition from the global coordinate system ($x \hspace{1pt} y \hspace{1pt} z$) to any arbitrary local coordinate system ($\dddot{x} \hspace{1pt} \dddot{y} \hspace{1pt} \dddot{z}$) is possible. The red rectangles show the rotation planes at three rotation steps.}
\label{fig:SystemModel}
\end{figure}







\begin{figure}[t]
	\centering
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \scalebox{0.25}{\includegraphics[trim={0.68cm 0.6cm 2.3cm 1.5cm},clip]{Fig1_MisA_0078.eps}}
        %\caption{$\mathbb{D}^{\Xi}$ with  $70,000$ samples}
        \label{Fig:_MisDE}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \scalebox{0.25}{
    		\includegraphics[trim={0.68cm 0.6cm 2.3cm 1.5cm},clip]{Fig1_MisA_0081.eps}}
        %\caption{$\mathbb{D}^{\Xi}_{10\%}$ with $7,000$ samples}
        \label{Fig:_MisDE10}
    \end{subfigure}
    ~ 
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \scalebox{0.25}{
    		\includegraphics[trim={0.68cm 0.6cm 2.3cm 1.5cm},clip]{Fig1_MisA_0082.eps}}
        %\caption{$\mathbb{D}^{\Xi}_{1\%}$ with $700$ samples}
        \label{Fig:_MisDE1}
    \end{subfigure}
    
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \scalebox{0.25}{\includegraphics[trim={0.8cm 0.6cm 2.3cm 1.5cm},clip]{Fig1_ESE_0078.eps}}
        \caption{$\mathbb{D}^{\Xi}$ with  $70,000$ samples}
        \label{Fig:_SEDE}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \scalebox{0.25}{
    		\includegraphics[trim={0.8cm 0.6cm 2.3cm 1.5cm},clip]{Fig1_ESE_0081.eps}}
        \caption{$\mathbb{D}^{\Xi}_{10\%}$ with $7,000$ samples}
        \label{Fig:_SEDE10}
    \end{subfigure}
    ~ 
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \scalebox{0.25}{
    		\includegraphics[trim={0.8cm 0.6cm 2.3cm 1.5cm},clip]{Fig1_ESE_0082.eps}}
        \caption{$\mathbb{D}^{\Xi}_{1\%}$ with $700$ samples}
        \label{Fig:_SEDE1}
    \end{subfigure}
    
	\caption{Misalignment probability and effective spectral efficiency for different dataset sizes}
	\label{Fig:DiffDatasets}
\end{figure}

